BitPrefill: W1.58A4 Tensor-Core Acceleration for Compute-Bound LLM Prefill

Low-bit quantization reduces large language model (LLM) inference cost, yet implementations optimized for memory-bound decode can leave compute-bound prefill on BF16 tensor cores. This gap matters for input-heavy workloads, including long-context and multimodal applications, where prefill can account for a substantial fraction of inference latency. We propose a W1.58A4 operator that quantizes weights to ternary values and activations to 4-bit, while executing the linear projection on native INT4 general matrix multiply (GEMM) tensor cores, turning prefill from a full-precision matrix multiply into a low-bit one. We deploy the operator for BitNet-b1.58 on a single RTX 4090 and a Jetson Orin Nano edge device, and report GEMM-kernel latency, end-to-end LLMs prefill latency, and task accuracy against bf16 and BitNet/BitBLAS baselines. Our proposed kernel achieves ~1.42x acceleration compared to the original BF16 prefill phase, with negligible reduction on model accuracy.

==> date_2027/2_related_work.tex <==
\section{Related Work}

\subsection{Low-bit Large Language Models}
 BitNet~\cite{bitnet} showed that a transformer can be trained end-to-end with 1-bit weights through a quantization-aware BitLinear layer, and BitNet-b1.58~\cite{bitnet1_58} relaxed this to ternary weights with absmean scaling, matching full-precision perplexity at scale.
 The open BitNet-b1.58-2B4T~\cite{bitnetb1_58-2b4t} is the largest public model of this family.
 Spectra~\cite{spectra} and ParetoQ~\cite{paretoq} confirm that ternary models sit on the size-accuracy Pareto frontier above B parameters, while PB-LLM~\cite{pbllm}, BiLLM~\cite{billm} and OneBit~\cite{onebit} reach the 1-bit regime from a pretrained model.
 All of these quantize only the weights, while activations stay at 8 or 16 bits, so the GEMM kernel still runs at INT8/BF16 precision and the prefill compute roofline is untouched.
 The closest work to ours, BitNet a4.8~\cite{bitnet_a4_8}, brings 4-bit activations to ternary LLMs with a hybrid quantization/sparsification recipe and a two-stage 8-to-4-bit training schedule, but it is an algorithmic result without a released GPU kernel.
 We provide the INT4 tensor-core operator such a W1.58A4 model needs and measure it end-to-end on a consumer GPU and an edge device.

 On the systems side, bitnet.cpp~\cite{bitnet_cpp} is the official CPU engine for ternary LLMs.
 It builds on T-MAC~\cite{tmac}'s table-lookup formulation, which precomputes partial sums of grouped low-bit weights so mixed-precision GEMM runs without dequantization, and LUT Tensor Core~\cite{luttensorcore} extends the idea into a hardware/software co-design.
 These target the memory-bound, low-decode regime on CPU SIMD or custom hardware.
 We target the compute-bound, large-prefill regime on commodity GPU tensor cores, a complementary point in the serving design space.



\subsection{GEMM Kernels for Low-bit LLMs}
 A low-bit LLM is only as fast as the GEMM kernel that consumes its quantized operands. 
 CUTLASS~\cite{cutlass}, NVIDIA's C++ template library, composes a GEMM kernel from compile-time building blocks-threadblock/warp/instruction tile shapes, a multi-stage \texttt{cp.async} pipeline and a threadblock swizzle, which is the open path to the native INT4 MMA on Ampere/Ada GPUs.
 Because tile shapes are template parameters, a library instantiates a table of kernels and selects one at runtime, and its classic epilogue is a fixed affine functor.
 BitBLAS~\cite{bitblas} takes the compiler route instead.
 Built on Ladder's type system, it lowers mixed-precision GEMMs (FP16xINT4, INT8xINT4, INT4xINT4, etc.) through TVM with per-shape JIT autotuning, and offers a fixed menu of weight-centric fusions.
 The Epilogue Visitor Tree (EVT)~\cite{evt} extends CUTLASS's epilogue into a compile-time tree of visitor nodes, accumulator fetch, row/column broadcast, element-wise compute, reductions, auxiliary loads and stores, traversed while the output tile is still in registers, with a thread layout derived from the GEMM tile shape so that fusion composes with tile selection.
 We build on CUTLASS with EVT: it reaches the INT4 MMA, selects tiles ahead of time without a JIT, and lets us express the two-sided per-token/per-channel dequantization as a fused epilogue, which BitBLAS's fixed menu cannot.

\subsection{Quantization-Aware Training and Post-Training Quantization}
Post-training quantization (PTQ) converts a pretrained LLM to low precision without end-to-end retraining, typically using only a small calibration set. Weight-only methods have shown that LLM weights can be compressed aggressively while retaining model quality. GPTQ~\cite{gptq} uses approximate second-order information to compensate quantization error and enables accurate 3--4-bit weight quantization, while AWQ~\cite{awq} identifies salient weights from activation statistics and applies channel-wise scaling to improve hardware-friendly low-bit weight-only inference. When activations are also quantized, however, large activation outliers become a major source of error. SmoothQuant~\cite{smoothquant} addresses this problem by migrating quantization difficulty from activations to weights through an equivalent channel-wise rescaling, enabling W8A8 inference. More recent rotation-based PTQ methods target even lower precision: QuaRot~\cite{quarot} uses orthogonal rotations to suppress activation outliers and enables end-to-end 4-bit quantization of weights, activations, and the KV cache, while SpinQuant~\cite{spinquant} learns such rotations to further improve low-bit accuracy.

Quantization-aware training (QAT), in contrast, exposes the model to quantization during optimization so that its parameters can adapt to the resulting discretization error. Since rounding is non-differentiable, QAT commonly employs the straight-through estimator (STE)~\cite{ste} during backpropagation. For LLMs, LLM-QAT~\cite{llmqat} combines data-free distillation with QAT and jointly quantizes weights, activations, and the KV cache down to 4 bits. EfficientQAT~\cite{efficientqat} reduces the otherwise substantial training cost of LLM QAT through block-wise optimization of model parameters followed by end-to-end optimization of quantization parameters, demonstrating effective quantization even in 2--3-bit weight regimes. BitNet~\cite{bitnet} and BitNet~b1.58~\cite{bitnet158} take a more aggressive approach by incorporating low-bit weights directly into model training; in particular, BitNet~b1.58 constrains weights to the ternary set ${-1,0,1}$ rather than converting a pretrained dense weight matrix after training.

==> date_2027/3_method.tex <==
\section{The Proposed Method}
 A BitNet-b1.58 linear layer computes $Y = XW^T$ with activations $X \in \mathbb{R}^{M \times K}$ and weights $W \in \mathbb{R}^{N \times K}$, where $M$ is the number of tokens processed in one forward pass.
 %
 Prefill processes the whole prompt at once ($M$=prompt length), decode one token per step ($M=1$).
 %
 We execute the prefill process projection by packing a ternary weight into a single INT4 as the INT4xINT4 tensor-core GEMM whose dequantization is fused into the epilogue, while keep the decode as the original ternary weight GEMV.
 %
 Section~\ref{sec: quantization and packing} describes the W4A4 quantization scheme and how weights and activations are packed for the INT4 tensor-core path.
 %
 Section~\ref{sec: autotuned gemm} describes the INT4 GEMM itself: a table of tile configurations compiled ahead of time, selected per problem shape at runtime, and scheduled with Stream-K.
 %
 Section~\ref{sec: evt-fused dequantization} describes the EVT epilogue that folds per-channel and per-token dequantization into the GEMM and emits bf16 directly.
 \TODO{Figure 1 [TODO] shows the operator end to end: quantize/pack → INT4 GEMM → EVT dequant → bf16.}

\subsection{W4A4 Quantization and Packing}
\label{sec: quantization and packing}
 For the GEMM operator, arithmetic intensity is:
\begin{equation}
\begin{aligned}
 I(M) = \frac{2MNK}{b_aMK + b_wNK + b_oMN}[ops/byte],
\end{aligned}
\end{equation} $b_a, b_w, b_o$ denote the bytes per activation, weight and output element.
 %
 For $M=1$, $I \approx 2/b_w$, i.e., decode is memory-bound and only the wight bytes $b_w$ matters, that is, weight-only quantization is enough there.
 %
 For $M \gg N$, $I \approx 2N/(b_a+b_o)$ grows with activations size, so prefill is compute-bound and its speed is set by the precision of the multiply-accumulate itself.
 % For the prefill GEMM to run on integer tensor cores, both operands must be integers of the same low width; quantizing only the weights leaves the multiply-accumulate in BF16. We therefore quantize weights and activations to signed 4-bit and pack them into the layout the INT4 MMA expects.

 \paragraph{Weight ternarization}
 Following BitNet-b1.58, weights are ternarized with absmean scaling.
 %
 With a per-output-channel scale,
\begin{equation}
\begin{aligned}
\label{eq: weight quantization}
 \alpha_n &= \frac{1}{K}\sum_{k=1}^K[W_{n,k}], \\ \tilde{W}_{n,k} &= clip (round(\frac{W_{n,k}}{\alpha_n}, -1, 1)),
\end{aligned}
\end{equation}where $W_{n,k} \approx \alpha_n\tilde{W}_{n,k}$ with $\tilde{W}_{n,k} \in {-1, 0, 1}$.
 %
 The ternary values are a subset of signed INT4; each is stored in a 4-bit two's-complement field.
 %
 W1.58 is the algorithmic precision, INT4 the physical container demanded by the INT4xINT4 tensor core: Ampere/Ada expose no INT2 MMA, and because prefill is compute-bound the two idle bits per weight cost no throughput.

 \paragraph{Activation quantization} Activations are quantized per token with a symmetric absmax quantizer to the INT4 range $[-8, 7]$:
\begin{equation}
\begin{aligned}
\label{eq: activation quantization}
 s_m &= \frac{7}{max(max_k[X_{m,k}], c)}, \\X_{m.k}^q &= clip(round(s_mX_{m,k}), -8, 7).
\end{aligned}
\end{equation}where $X_{m,k} \approx X_{m,k}^q/s_m$.
 Per-token granularity needs no calibration set and no rotation.
 Unlike Hadamard-based W4A4 schemes~\cite{bitnet_a4_8}, nothing has to be folded into the ternary weights.

 \paragraph{Integer GEMM and dequantization} The tensor core computes the exact integer product and accumulates in INT32,
\begin{equation}
\begin{aligned}
 acc_{m,n} = \sum_{k=1}^K X_{m,k}^q\tilde{W}_{n,k} \in \mathbb{Z}, \quad |acc_{m,n} \leq 8K|,
\end{aligned}
\end{equation}and the output is recovered by a two-sided rescale:
\begin{equation}
\begin{aligned}
 Y_{m,n} \approx \frac{\alpha_n}{s_m}acc_{m,n}.
\end{aligned}
\end{equation}

\paragraph{Packing} Two INT4 fields share one byte: element $k$ occupies byte $[k/2]$, even $k$ in the low nibble, odd $k$ in the high nibble.
 %
 Thus $W \in \mathbb{R}^{N \times K}$ is stored as $N \times K/2$ bytes and $X$ as $M \times K/2$ bytes, both plain row-major for CUTLASS operand iterators.

\subsection{Shape-Adaptive INT4 GEMM Execution}
\label{sec: autotuned gemm}
\paragraph{Wave quantization} A data-parallel GEMM with threadblock tile $T_M \times T_N$ launches:
\begin{equation}
\begin{aligned}
 n_{tile} = \lceil\frac{M}{T_M}\rceil\lceil\frac{N}{T_N}\rceil
\end{aligned}
\end{equation}threadblocks, one per output tile.
%
 On P streaming multiprocessors they execute in $\lceil n_{tile}/P \rceil$ waves, so the SM utilization is:
\begin{equation}
\begin{aligned}
 \eta(T_M, T_N) = \frac{n_{tile}}{P\lceil n_{tile}/P \rceil}.
\end{aligned}
\end{equation} The partial final wave costs as much as a full one. 
%
 Which tile maximizes $\eta$ (and balances it against per-tile efficiency, which favors large tiles) depends on $M$, and $M$ varies across layers and prompts in prefill.
%
 CUTLASS tile shapes, however, are compile-time template parameters and cannot follow a runtime $(M, N, K)$.

 
\paragraph{Pre-compiled candidates, per-shape selection} We separate compilation from selection.
%
A kernel configuration is the tuple:
\begin{equation}
\begin{aligned}
\label{eq: shape cadidate}
 c=(T_M, T_N, W_M, W_N, S),
\end{aligned}
\end{equation}where $T_M \times T_N$ is the threadblock tile.
%
 $W_M \times W_N$ is the warp tile, the sub-block of that tile each of the $(T_M/W_M)(T_N/W_N)$ warps accumulates in registers, which trades register pressure against operand reuse from shared memory.
 $S$ denotes the number of $K$-slices are in flight between global and shared memory, hiding load latency at the cost of $S$ shared-memory buffers.
%
 The first call for a shape measures every candidate on the kernel-level and caches:
\begin{equation}
\begin{aligned}
 c^*(M,N,K) = \arg\min_{c \in C} t_c(M, N, K),
\end{aligned}
\end{equation}after which calls dispatch directly to $c^*$.

 \paragraph{Stream-K scheduling.} Data-parallel scheduling fixes the tile count $n_{tile}$, so a tile count that is not a multiple of the streaming multiprocessor (SM) count will leave a partial final wave that still costs a full wave.
 We apply Stream-K~\cite{streamk} instead flattens the GEMM into its mainloop iterations and gives every block an equal slice, reconciling partial tiles through a workspace and a semaphore; this keeps the SMs balanced in exactly the small- and irregular-M regimes where prefill lives.
 % The live operator is initialized once per (shape, pointers) and re-run, so the steady-state path pays no re-initialization memset.
 % Pre-compilation lookup table plus Stream-K gives one operator that stays near the best tile choice across the whole prefill $M$-range, rather than a heuristic that is optimal at one $M$ and wasteful at others.

\subsection{EVT-Fused Dequantization Epilogue}
\label{sec: evt-fused dequantization}
 \TODO{Show Figure: The visitor chain is $AccFetch \rightarrow \times col\_scale (row~broadcast) \rightarrow \times 1/row\_scale (column~broadcast) \rightarrow store bf16$.}
 An INT4 GEMM produces an INT32 accumulator, but the model needs BF16 scaled by the per-channel weight scale and the per-token activation scale.
 Performed as a separate kernel after the GEMM, this de-quantization reads and writes the full $M \times N$ output several times — an extra memory-bound pass whose cost is significant precisely:
\begin{equation}
\begin{aligned}
 B_{unfused} &= \underbrace{4MN}_{\text{store acc}} + \underbrace{4MN}_{\text{load acc}} + \underbrace{2MN}_{\text{store Y}} = 10 MN \; bytes, \\
 B_{fused} &= 2MN \; bytes.
\end{aligned}
\end{equation} Because the INT4 GEMM is several times faster than its BF16 counterpart, this output-side traffic is no longer negligible relative to the compute it follows.

 We express the de-quantization as an Epilogue Visitor Tree (EVT) and fuse it into the GEMM's store stage.
 The epilogue computes:
\begin{equation}
\begin{aligned}
 D_{m,n} = bf16(acc_{m,n} \times \frac{\alpha_n}{s_m}), \\
 
\end{aligned}
\end{equation}where $\alpha_n$ is the per-output-channel weight scale broadcast down $M$, and $s_m$ is the per-token (inverse) activation scale broadcast across $N$, as shown in Eq.~\ref{eq: weight quantization} and Eq.~\ref{eq: activation quantization}.
 %
 The two scale vectors are tiny and align with the tile a threadblock already owns ($\alpha$ with its $N$-slice, $s$ with its $M$-slice), so they are read once into on-chip memory and reused across the tile.
 %
 The accumulator is rescaled in registers immediately after the MMA and the INT32 result never reaches HBM.
 Since EVT derives its thread layout from the GEMM tile shape, the same tree is instantiated for every candidate in Eq.~\ref{eq: shape cadidate}.
 %
 Fusion removes the INT32 round-trip entirely: the accumulator is scaled in registers and only BF16 is written back, halving the output bytes and collapsing several dequantization passes into the GEMM's single store.
 
